The LUNIS-AGN Catalog: Trends of emission line velocity dispersion and surface brightness within the circumnuclear regions of Seyfert galaxies

We present a catalog of Local Universe Near-Infrared Seyfert (LUNIS) \textit{K-}band integral field unit (IFU) data of 88 nearby Active Galactic Nuclei (AGN), curated from SINFONI/VLT and OSIRIS/Keck archival datasets. This catalog includes both type 1 and 2 Seyfert AGN probed down to scales of tens of parsecs with z $<$ 0.02 and spanning over five orders of magnitude in L$_{14-195keV}$ AGN luminosity. As part of this catalog we make publicly available for all galaxies the processed datacubes, a central 200 pc integrated spectrum, and two-dimensional maps of flux, velocity, and velocity dispersion for H$_2$ 1-0 S(1) 2.1218 $\mu$m, [Si VI] 1.9641 $\mu$m, and Br-$\gamma$ 2.1655 $\mu$m. The morphology and geometry of [Si VI], a tracer of AGN outflows, are reported for the 66$\%$ of galaxies with extended emission. We utilize this large sample to probe the behavior of molecular and ionized gas, identifying trends in the properties of the circumnuclear gas (surface brightness and velocity dispersion) with fundamental AGN properties (obscuration and X-ray luminosity). While there is significant variation in circumnuclear gas characteristics across the sample, we find molecular hydrogen to be less centrally concentrated and exhibit lower velocity dispersion relative to ionized gas. In addition, we find elevated molecular hydrogen surface brightness and decreased [Si VI] velocity dispersion in obscured relative to unobscured AGN. The [Si VI] and Br-$\gamma$ emission scale with L$_{14-195keV}$ X-ray luminosity, which, along with the elevated velocity dispersion compared to the molecular gas, verifies an association with AGN outflow processes.

==> Latex_Table_Test.tex <==
\begin{tabular}{llllrr}
\toprule
       Galaxy &   Sample &         Type &          SWIFT\_ID &  pc\_arcsecond &  pc\_per\_pixel \\
\midrule
      NGC1365 &  SINFONI &       Sy 1.8 & SWIFTJ0333.6-3607 &     86.781706 &      4.339085 \\
      NGC2110 &  SINFONI &    Sy 2 (1h) & SWIFTJ0552.2-0727 &    172.593784 &      8.629689 \\
      NGC2992 &  SINFONI &       Sy 1.8 & SWIFTJ0945.6-1420 &    153.201224 &      7.660061 \\
      NGC3081 &  SINFONI &    Sy 2 (1h) & SWIFTJ0959.5-2248 &    128.475710 &      6.423786 \\
      NGC3783 &  SINFONI &       Sy 1.2 & SWIFTJ1139.0-3743 &    231.741092 &     11.587055 \\
      NGC4593 &  SINFONI &   Sy 1.0-1.2 & SWIFTJ1239.6-0519 &    128.960524 &      6.448026 \\
      NGC5506 &  SINFONI &    Sy 2 (1i) & SWIFTJ1413.2-0312 &    115.385732 &      5.769287 \\
      NGC5728 &  SINFONI &         Sy 2 & SWIFTJ1442.5-1715 &    129.930152 &      6.496508 \\
      NGC6814 &  SINFONI &       Sy 1.5 & SWIFTJ1942.6-1024 &    110.537592 &      5.526880 \\
      NGC7172 &  SINFONI &    Sy 2 (1i) & SWIFTJ2201.9-3152 &    164.351946 &      8.217597 \\
      NGC7582 &  SINFONI &    Sy 2 (1i) & SWIFTJ2318.4-4223 &    101.326126 &      5.066306 \\
  eso137-G034 &  SINFONI &         Sy 2 & SWIFTJ1635.0-5804 &    185.000000 &      9.250000 \\
MCG-05-23-016 &  SINFONI &       Sy 1.9 & SWIFTJ0947.6-3057 &    168.000000 &      8.400000 \\
MCG-06-30-015 &  SINFONI &       Sy 1.2 & SWIFTJ1335.8-3416 &    130.000000 &     16.250000 \\
      ic4329a &     KONA &         Sy1  & SWIFTJ1349.3-3018 &    321.000000 &     11.235000 \\
    iras01475 &     KONA &         Sy1h &               NaN &    354.000000 &     17.700000 \\
       mrk573 &     KONA &         Sy1h &               NaN &    346.000000 &     12.110000 \\
       mrk766 &     KONA &         Sy1  & SWIFTJ1218.5+2952 &    266.000000 &     13.300000 \\
      ngc4151 &     KONA &         Sy1  & SWIFTJ1210.5+3924 &     66.000000 &      2.310000 \\
       ngc262 &     KONA &         Sy1h & SWIFTJ0048.8+3155 &    311.000000 &     10.885000 \\
       ngc513 &     KONA &         Sy1h & SWIFTJ0124.5+3350 &    390.000000 &     19.500000 \\
       ngc591 &     KONA &         Sy1h &               NaN &    310.000000 &     15.500000 \\
      ngc1194 &     KONA &         Sy2  & SWIFTJ0304.1-0108 &    268.000000 &     13.400000 \\
      ngc3516 &     KONA &         Sy1  & SWIFTJ1106.5+7234 &    177.000000 &      6.195000 \\
      ngc4051 &     KONA &   Sy1 / Sy1n & SWIFTJ1203.0+4433 &     64.500000 &      2.257500 \\
      ngc4388 &     KONA &         Sy1h & SWIFTJ1225.8+1240 &    103.800000 &      5.190000 \\
      ngc4748 &     KONA &         Sy1  & SWIFTJ1252.3-1323 &    278.000000 &      9.730000 \\
      ngc5548 &     KONA &         Sy1  & SWIFTJ1417.9+2507 &    345.000000 &     12.075000 \\
      ngc7682 &     KONA &        Sy1h  &               NaN &    343.000000 &     17.150000 \\
       ESO548 & SINFONI2 &         Sey1 & SWIFTJ0342.0-2115 &    284.000000 &     14.200000 \\
       IC1459 & SINFONI2 &        LINER &               NaN &    137.700000 &      6.885000 \\
       IC5267 & SINFONI2 &      Not AGN &               NaN &    111.000000 &     13.875000 \\
       NGC357 & SINFONI2 &      Not AGN &               NaN &    158.000000 &     19.750000 \\
       NGC613 & SINFONI2 &            ? &               NaN &     99.000000 &      4.950000 \\
      NGC1052 & SINFONI2 &        Sey3h & SWIFTJ0241.3-0816 &     97.000000 &      4.850000 \\
      NGC1566 & SINFONI2 &       Sey1.5 & SWIFTJ0420.0-5457 &     59.100000 &      2.955000 \\
      NGC1614 & SINFONI2 &         Sey2 &               NaN &    314.600000 &     39.325000 \\
      NGC2974 & SINFONI2 &         Sey2 &               NaN &    119.700000 &      5.985000 \\
      NGC3227 & SINFONI2 &       Sey1.5 & SWIFTJ1023.5+1952 &    101.300000 &      1.266250 \\
      NGC3312 & SINFONI2 &         Sey3 &               NaN &    216.700000 &     10.835000 \\
      NGC4030 & SINFONI2 &      Not AGN &               NaN &     97.000000 &     12.125000 \\
      NGC4261 & SINFONI2 &        Sey3h &               NaN &    142.500000 &     17.812500 \\
      NGC7496 & SINFONI2 &         Sey2 &               NaN &     72.700000 &      3.635000 \\
       IC5063 & SINFONI2 &        Sey1h & SWIFTJ2052.0-5704 &    202.200000 &     10.110000 \\
          M87 & SINFONI2 &        LINER &               NaN &     82.903194 &      4.145160 \\
       MCG523 & SINFONI2 &            0 &               NaN &    168.000000 &      8.400000 \\
       NGC289 & SINFONI2 &            0 &               NaN &    107.000000 &      5.350000 \\
       NGC628 & SINFONI2 &      Not AGN &               NaN &     44.000000 &      5.500000 \\
       NGC676 & SINFONI2 &         Sey2 &               NaN &     94.538730 &      4.726937 \\
      NGC1068 & SINFONI2 &        Sey1h & SWIFTJ0242.6+0000 &     69.813216 &      3.490661 \\
      NGC1097 & SINFONI2 &        Sey3b &               NaN &     82.418380 &      4.120919 \\
      NGC1386 & SINFONI2 &        Sey1i &               NaN &     78.539868 &      3.926993 \\
      NGC2911 & SINFONI2 &         Sey3 &               NaN &    252.103280 &     12.605164 \\
      NGC3125 & SINFONI2 &    2 I Think &               NaN &     73.000000 &      9.125000 \\
      NGC3169 & SINFONI2 &        LINER &               NaN &     91.145032 &      4.557252 \\
      NGC3281 & SINFONI2 &         Sey2 & SWIFTJ1031.7-3451 &    236.104418 &     11.805221 \\
      NGC3368 & SINFONI2 &        LINER &               NaN &     52.359912 &      2.617996 \\
      NGC3621 & SINFONI2 &            0 &               NaN &     48.000000 &      0.600000 \\
      NGC3627 & SINFONI2 &         Sey3 &               NaN &     31.997724 &      1.599886 \\
      NGC4303 & SINFONI2 &         Sey2 &               NaN &     73.691728 &      9.211466 \\
      NGC4438 & SINFONI2 &        Sey3b &               NaN &     67.389146 &      3.369457 \\
      NGC4472 & SINFONI2 &   Sey2 LINER &               NaN &     82.903194 &     10.362899 \\
      NGC4569 & SINFONI2 &        LINER &               NaN &     60.116936 &      3.005847 \\
      NGC4579 & SINFONI2 &        Sey3b &               NaN &     81.448752 &      4.072438 \\
      NGC4762 & SINFONI2 &        LINER &               NaN &     81.448752 &      4.072438 \\
      NGC4945 & SINFONI2 &         Sey2 & SWIFTJ1305.4-4928 &     18.810783 &      0.940539 \\
      NGC5128 & SINFONI2 &         Sey2 &               NaN &     18.422932 &      0.230287 \\
      NGC5135 & SINFONI2 &         Sey2 &               NaN &    295.251726 &     36.906466 \\
      NGC6300 & SINFONI2 &         Sey2 & SWIFTJ1717.1-6249 &     65.934704 &      8.241838 \\
      NGC7130 & SINFONI2 &       Sey1.9 & SWIFTJ2148.3-3454 &    308.341704 &     38.542713 \\
      NGC7135 & SINFONI2 &          AGN &               NaN &    173.000000 &      8.650000 \\
      NGC7213 & SINFONI2 & LINER Sey1.5 & SWIFTJ2209.4-4711 &    106.659080 &      5.332954 \\
      NGC7469 & SINFONI2 &       Sey1.5 & SWIFTJ2303.3+0852 &    274.889538 &      3.436119 \\
      NGC7743 & SINFONI2 &         Sey2 &               NaN &     93.084288 &     11.635536 \\
       ARP220 & SINFONI2 &   LINER Sey2 &               NaN &    365.549756 &     18.277488 \\
     Circinus & SINFONI2 &        Sey1h &               NaN &     20.362188 &      0.254527 \\
      NGC5643 & SINFONI2 &         Sey2 & SWIFTJ1432.8-4412 &     81.933566 &     10.241696 \\
      NGC4501 & SINFONI2 &         Sey2 &               NaN &     81.448752 &      4.072438 \\
      mrk1066 &     KONA &         Sy2  &               NaN &    240.000000 &     12.000000 \\
      mrk1210 &     KONA &         Sy2  & SWIFTJ0804.2+0507 &    281.000000 &      9.835000 \\
      ngc1320 &     KONA &         Sy2  &               NaN &    178.000000 &      8.900000 \\
      ngc1667 &     KONA &         Sy2  &               NaN &    315.000000 &     11.025000 \\
      ngc3393 &     KONA &         Sy2  & SWIFTJ1048.4-2511 &    255.000000 &     12.750000 \\
      ngc6967 &     KONA &         Sy2  &               NaN &    252.000000 &      8.820000 \\
      ngc7465 &     KONA &         Sy2  & SWIFTJ2302.1+1557 &    130.000000 &      4.550000 \\
       ESO428 & SINFONI2 &            2 &               NaN &    117.809802 &      5.599602 \\
         Mrk9 &   OSIRIS &          NaN & SWIFTJ0736.9+5846 &           NaN &           NaN \\
         Mrk3 &   OSIRIS &          NaN & SWIFTJ0615.8+7101 &           NaN &           NaN \\
     NGC 1358 &   OSIRIS &          NaN &               NaN &           NaN &           NaN \\
          M81 &   OSIRIS &          NaN & SWIFTJ0955.5+6907 &           NaN &           NaN \\
         M104 &  SINFONI &          NaN &               NaN &           NaN &           NaN \\
      NGC1204 &   OSIRIS &          NaN &               NaN &           NaN &           NaN \\
         3C84 &   OSIRIS &          NaN &               NaN &           NaN &           NaN \\
       IC2560 &  SINFONI &          NaN &               NaN &           NaN &           NaN \\
       IC4995 &  SINFONI &          NaN &               NaN &           NaN &           NaN \\
          M84 &  SINFONI &          NaN &               NaN &           NaN &           NaN \\
      NGC1808 &  SINFONI &          NaN &               NaN &           NaN &           NaN \\
      NGC1672 &  SINFONI &          NaN &               NaN &           NaN &           NaN \\
       NGC253 &  SINFONI &          NaN &               NaN &           NaN &           NaN \\
          M64 &  SINFONI &          NaN &               NaN &           NaN &           NaN \\
       NGC404 &   OSIRIS &          NaN &               NaN &           NaN &           NaN \\
      NGC7217 &   OSIRIS &          NaN &               NaN &           NaN &           NaN \\
      NGC5953 &   OSIRIS &          NaN &               NaN &           NaN &           NaN \\
          M94 &   OSIRIS &          NaN &               NaN &           NaN &           NaN \\
      NGC3998 &   OSIRIS &          NaN & SWIFTJ1157.8+5529 &           NaN &           NaN \\
      NGC7591 &   OSIRIS &          NaN &               NaN &           NaN &           NaN \\
       IC4296 &  SINFONI &          NaN &               NaN &           NaN &           NaN \\
      NGC4643 &  SINFONI &          NaN &               NaN &           NaN &           NaN \\
      NGC6328 &  SINFONI &          NaN &               NaN &           NaN &           NaN \\
      NGC7410 &  SINFONI &          NaN &               NaN &           NaN &           NaN \\
       NGC315 &   OSIRIS &          NaN &               NaN &           NaN &           NaN \\
      NGC4450 &  SINFONI &          NaN &               NaN &           NaN &           NaN \\
      NGC4636 &  SINFONI &          NaN &               NaN &           NaN &           NaN \\
\bottomrule
\end{tabular}

